Impact of Aliasing on Generalization in Deep Convolutional Networks

We investigate the impact of aliasing on generalization in Deep Convolutional Networks and show that data augmentation schemes alone are unable to prevent it due to structural limitations in widely used architectures. Drawing insights from frequency analysis theory, we take a closer look at ResNet and EfficientNet architectures and review the trade-off between aliasing and information loss in each of their major components. We show how to mitigate aliasing by inserting non-trainable low-pass filters at key locations, particularly where networks lack the capacity to learn them. These simple architectural changes lead to substantial improvements in generalization on i.i.d. and even more on out-of-distribution conditions, such as image classification under natural corruptions on ImageNet-C [11] and few-shot learning on Meta-Dataset [26]. State-of-the art results are achieved on both datasets without introducing additional trainable parameters and using the default hyper-parameters of open source codebases.

==> tables/imagenet_iid_combinations.tex <==
{\setlength{\tabcolsep}{0.1em}
\begin{table}[h]
\scriptsize
\begin{center}
\begin{tabular}{@{}lccccccc@{}}
  \toprule
  & \multicolumn{3}{c}{Blur before} && \multicolumn{3}{c}{Blur after} \\
  \cmidrule{2-4} \cmidrule{6-8}
  Combination & $k=3$ & $k=5$ & $k=7$ && $k=3$ & $k=5$ & $k=7$ \\
  \midrule
  \DTLforeach{imagenet_iid_combinations}{%
    \method=Method,%
    \bbthree=BB3,%
    \bbfive=BB5,%
    \bbseven=BB7,%
    \bathree=BA3,%
    \bafive=BA5,%
    \baseven=BA7%
  }{%
    \DTLiffirstrow{}{\\}%
    \dtlformat{\method}&%
    \dtlformat{\bbthree}&%
    \dtlformat{\bbfive}&%
    \dtlformat{\bbseven}&&%
    \dtlformat{\bathree}&%
    \dtlformat{\bafive}&%
    \dtlformat{\baseven}
  }
  \\ \bottomrule
\end{tabular}
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
%  \multicolumn{1}{c}{} & 
%   \multicolumn{3}{c}{blur before} &
%   \multicolumn{3}{c}{blur after}  \\ 
% filter size & 3 & 5 & 7 & 3 & 5 & 7 \\  
% subsampled &
% \\ 
% subsampled low capacity & 

% \end{tabular}
\end{center}
\caption{\label{table:imagenet_iid_combinations} Imagenet results: combining anti-aliasing sub-sampling modules. Impact of anti-aliasing modules that don't have capacity to learn anti-alias versus all sub-sampled modules. MAYBE A PLOT HERE
}
\end{table}
}

==> tables/imagenet_iid_combinations_strong.tex <==
{\setlength{\tabcolsep}{0.1em}
\begin{table}[ht]
\scriptsize
\begin{center}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multicolumn{3}{c}{Blur filter location} & \phantom{a} & \multicolumn{2}{c}{Blur before {\tiny(filter size $k$)}} & \phantom{a} & \multicolumn{2}{c}{Blur after {\tiny(filter size $k$)}} \\
\cmidrule{1-3} \cmidrule{5-6} \cmidrule{8-9}
skip & max-pool & block-conv && $k=3$ & $k=5$ && $k=3$ & $k=5$ \\
\midrule
\checkmark &            &            && 78.55 {\tiny $\pm$ 0.05} & 78.65 {\tiny $\pm$ 0.13} && 78.54 {\tiny $\pm$ 0.03} & 78.60 {\tiny $\pm$ 0.17} \\
\checkmark & \checkmark &            && 78.68 {\tiny $\pm$ 0.14} & 78.65 {\tiny $\pm$ 0.07} && 78.61 {\tiny $\pm$ 0.14} & 78.57 {\tiny $\pm$ 0.10} \\
\checkmark &            & \checkmark && 78.92 {\tiny $\pm$ 0.02} & 78.84 {\tiny $\pm$ 0.04} && 78.87 {\tiny $\pm$ 0.07} & 78.94 {\tiny $\pm$ 0.02} \\
\checkmark & \checkmark & \checkmark && 78.85 {\tiny $\pm$ 0.13} & 78.80 {\tiny $\pm$ 0.14} && 78.85 {\tiny $\pm$ 0.02} & 78.72 {\tiny $\pm$ 0.03} \\
\midrule
\multicolumn{6}{l}{Baseline {\tiny (ResNet-50 + RandAugment + Swish, 180 epochs)}} & \multicolumn{3}{c}{77.38{\tiny $\pm$0.06}} \\
\bottomrule
\end{tabular}
% \begin{tabular}{c|c|c|c|c|c|c}


% \multicolumn{6}{l}{ResNet-50 (ours) + RandAugment + Swish (180 epochs)} & 77.38 +-0.06 \\ \hline
% skip & max-pool & block-conv & 
% \multicolumn{4}{c}{filter size}
% \\
%  &  &  & 
% \multicolumn{2}{c}{blur before}
% \multicolumn{2}{c}{blur after}
% \\
%  \hline
%  & & &
%  \multicolumn{1}{c}{3}&
%  \multicolumn{1}{c}{5}&
%  \multicolumn{1}{c}{3}&
%  \multicolumn{1}{c}{5}
%  \\ \hline

% %skip only
%  \checkmark  & & &
% 78.55 +- 0.05 & 
% 78.65 +- 0.13  &
% 78.54 +- 0.03 &
% 78.60 +- 0.17 
% \\ \hline
%  %skip max

%  \checkmark   & \checkmark & &
%  78.68 +- 0.14 &
%  78.65 +- 0.07 &
%  78.61 +- 0.14 &
%  78.57 +- 0.10
%  \\ \hline
% %skip block 
%  \checkmark   & & \checkmark &
%  78.92 +-0.02 &
%  78.84 +-0.04 &
%  78.87 +-0.07 & 
%  78.94 +-0.02 
%  \\ \hline

%  \checkmark & \checkmark & \checkmark &
%  78.85 +- 0.13 &
%  78.80 +- 0.14 &
%  78.85 +- 0.02 & 
%  78.72 +- 0.03
%  \\ \hline
% \end{tabular}
\end{center}
\caption{\label{table:imagenet_iid_combinations_strong}ImageNet results when using data augmentation and smooth activations for various combinations of anti-aliasing locations. We see that all combinations reach higher accuracy than the baseline. Note that ``Blur before'' and ``Blur after'' only affect skip connections as anti-aliasing on max-pooling and block convolutions are fixed as ``Blur after''.
}
\end{table}
}


==> tables/meta_dataset_test_all.tex <==
{\setlength{\tabcolsep}{0.4em}
\begin{table*}[ht]
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccccccc@{}}
  \toprule
  & SUR* & \multicolumn{3}{c}{Blur skip + Conv1 w/stride 1} & GELU & \multicolumn{3}{c}{Blur all + Conv1 w/stride 1 + GELU } & \phantom{a} & \multicolumn{3}{c}{Blur skip + Conv1 w/stride 1 + GELU} \\ 
  \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
  Data source && $k=3$ & $k=5$ & $k=7$ && $k=3$ & $k=5$ & $k=7$ && $k=3$ & $k=5$ & $k=7$\\
  \midrule
  \DTLforeach{meta_dataset_test}{%
    \source=DATASOURCE,%
    \sur=SUR,%
    \surs=SUR-S,%
    \aasthree=AAS3,%
    \aasthrees=AAS3-S,%
    \aasfive=AAS5,%
    \aasfives=AAS5-S,%
    \aasseven=AAS7,%
    \aassevens=AAS7-S,%
    \gelu=GELU,%
    \gelus=GELU-S,%
    \aasubgthree=AASUBG3,%
    \aasubgthrees=AASUBG3-S,%
    \aasubgfive=AASUBG5,%
    \aasubgfives=AASUBG5-S,%
    \aasubgseven=AASUBG7,%
    \aasubgsevens=AASUBG7-S,%
    \aasgthree=AASG3,%
    \aasgthrees=AASG3-S,%
    \aasgfive=AASG5,%
    \aasgfives=AASG5-S,%
    \aasgseven=AASG7,%
    \aasgsevens=AASG7-S%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{%
    }{%
      \ifthenelse{\value{DTLrowi}=8 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \source&%
    \sur\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\surs}{}&%
    \aasthree\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasthrees}{}&%
    \aasfive\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasfives}{}&%
    \aasseven\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aassevens}{}&%
    \gelu\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\gelus}{}&%
    \aasubgthree\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasubgthrees}{}&%
    \aasubgfive\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasubgfives}{}&%
    \aasubgseven\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasubgsevens}{}&&%
    \aasgthree\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasgthrees}{}&%
    \aasgfive\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasgfives}{}&%
    \aasgseven\ifthenelse{\value{DTLrowi}<14}{\tiny$\pm$\aasgsevens}{}%
  }
  \\\bottomrule
\end{tabular}
% \begin{tabular}{l|cc|cccccc|cc|cccccc|cccccc}
%  \multicolumn{1}{c}{} & 
%   \multicolumn{2}{c}{SUR*} &
%   \multicolumn{6}{c}{A-A skip} & 
% \multicolumn{2}{c}{GELU} &
%   \multicolumn{6}{c}{A-A sub-sampled + GELU} & 
%       \multicolumn{6}{c}{A-A skip+ GELU} \\ 
% filter size & & & 3& & 5& &7 & & & & 3 & & 5 & & 7 & & 3 & & 5 && 7 \\ \hline 
% Imagenet &
% 53.77 & 1.1 &
% 57.32 & 1.13 & 58.46 & 1.08 & 58.67 & 1.09 &
% 56.81 & 1.11 & 
% 59.59 &  1.08 &  59.37 &  1.02 &  59.06 &  1.02 &
% 59.91 &  1.06 &  \textbf{60.59} &  1.04 &  58.03 &  1.07 \\ \hline 

% Omniglot &
% 95.81 & 0.36 &
% 96.11 & 0.36 & 95.87 & 0.36 & \textbf{96.45} & 0.33 &
% 96.29 & 0.32 & 
% 96.35 &  0.32 &  96.39 &  0.32 &  96.25 &  0.34 &
% 96.06 &  0.33 & \textbf{96.45} &  0.31 &  96.38 &  0.34 \\ \hline 

% Aircraft &
% 87.47 & 0.49 &
% 89.22 &  0.43 &  89.54 &  0.45 &  89.9 &  0.46 &
% 88.36 & 0.56 &
% \textbf{90.93} &  0.4 &  90.21 &  0.47 &  89.98 &  0.48 &
% 90.76 &  0.46 &  90.34 &  0.5 &  90.68 &  0.45 \\ \hline 

% Birds &
% 72.44 & 0.98 & 
% 78.7 &  0.87 &  77.86 &  0.82 &  77.36 &  0.9 &
% 72.81 & 0.89 &
% 79.52 &  0.81 &  \textbf{80.5} &  0.77 &  79.76 &  0.73 &
% 78.52 &  0.81 &  79.96 &  0.79 &  79.51 &  0.8 \\ \hline 

% Textures &
% 68.96 & 0.77 &
% 71.29 &  0.9 &  72.08 &  0.78 &  72.77 &  0.92 &
% 72.59 & 0.8 &
% \textbf{75.00} &  0.75 &  74.36 &  0.7 &  74.55 &  0.78 &
% 74.4 &  0.73 & 74.98 &  0.8 &  72.61 &  0.77 \\ \hline 

% Quick Draw &
% 81.58 & 0.6 &
% 82.3 &  0.54 &  82.29 &  0.56 &  82.29 &  0.59 &
% 83.05 & 0.54 &
% 83.81 &  0.53 &  83.23 &  0.56 &  83.58 &  0.52 &
% \textbf{84.01} &  0.54 &  83.18 &  0.53 &  82.88 &  0.57 \\ \hline 

% Fungi &
% 65.67 & 1.01 &
% 69.87 &  0.93 &  71.07 &  0.98 &  70.48 &  0.93 &
% 67.91 & 1.03 & 
% 72.99 &  0.95 &  \textbf{73.86} &  0.92 &  73.57 &  0.9 &
% 72.88 &  0.92 &  73.5 &  0.89 &  72.98 &  0.91 \\ \hline 

% VGG Flower &
% 87.61 & 0.63 &
% 89.04 &  0.55 &  87.69 &  0.6 &  89.25 &  0.58 &
% 87.55 & 0.58 &
% 90.55 &  0.47 &  \textbf{91.24} &  0.47 &  90.31 &  0.5 & 
% 88.81 &  0.52 &  89.31 &  0.48 &  90.09 &  0.51\\ \hline 

% Traffic Signs &
% 51.75 & 1.06 &
% 51.05 &  1.09 &  \textbf{55.52} &  1.03 &  52.15 &  1.07 &
% 53.51 & 1.06 &
% 54.17 &  1.0 &  51 &  1.02 &  51.96 &  0.99 &
% 51.55 &  1.01 &  53.51 &  1.04 &  49.11 &  1.0\\ \hline 

% MSCOCO &
% 48.95 & 1.1 &
% 48.3 &  1.09 &  49.61 &  1.05 &  47.34 &  1.09 &
% 49.71 & 1.05 &
% 49.53 &  1.05 &  49.55 &  1.01 &  49.38 &  1.02 &
% 50.28 &  1.04 &  \textbf{50.72} &  1.02 &  47.31 &  1.02 \\ \hline 

% MNIST &
% 94.04 & 0.49 &
% 92.9 &  0.55 &  92.11 &  0.56 &  88.06 &  0.51 &
% \textbf{95.42} & 0.43 &
% 94.13 &  0.46 &  89.77 &  0.5 &  94.05 &  0.47 &
% 93.84 &  0.51 &  91.02 &  0.45 &  92.46 &  0.44 \\ \hline 

% CIFAR10 &
% 62.45 & 0.91 &
% 66.22 &  0.84 &  66.06 &  0.85 &  62.32 &  0.93 &
% 63.2 & 1.01 &
% 68.45 &  0.74 &  68.21 &  0.78 &  66.44 &  0.77 &
% \textbf{69.6} &  0.77 &  69.29 &  0.71 &  63.75 &  0.8 \\ \hline 

% CIFAR100 &
% 53.12 & 1.1 &
% 56.89& 1.04 &  57.03 &  1.05 &  53.63 &  1.09 &
% 56.81 & 1.21 &
% 57.67 &  1.03 &  58.5 &  1.06 &  58.22 &  1.02 &
% \textbf{61.58} &  1.04 &  59.61 &  1.02 &  53.4 &  1.04 \\ \hline


% \multicolumn{1}{c}{Avg} & 
% \multicolumn{2}{c}{71.05} & 
% \multicolumn{2}{c}{73.02} &
% \multicolumn{2}{c}{73.48} & 
% \multicolumn{2}{c}{72.36} &   
% \multicolumn{2}{c}{72.62} &
% \multicolumn{2}{c}{ \textbf{74.82}} & 
% \multicolumn{2}{c}{74.32} &   
% \multicolumn{2}{c}{74.39} &
% \multicolumn{2}{c}{74.79} &
% \multicolumn{2}{c}{ \textbf{74.80}} & 
% \multicolumn{2}{c}{73.01} 
% \\ 
% \multicolumn{1}{c}{Avg in-domain } & 
% \multicolumn{2}{c}{76.66} &
% \multicolumn{2}{c}{79.23} & 
% \multicolumn{2}{c}{79.37} &   
% \multicolumn{2}{c}{79.65} &
% \multicolumn{2}{c}{78.17} &
% \multicolumn{2}{c}{81.09} & 
% \multicolumn{2}{c}{\textbf{81.15}} &   
% \multicolumn{2}{c}{80.88} &
% \multicolumn{2}{c}{80.67} & 
% \multicolumn{2}{c}{81.04} &   
% \multicolumn{2}{c}{80.40} 
% \\ 
% \multicolumn{1}{c}{Avg out-of-domain} & 
% \multicolumn{2}{c}{62.06} &
% \multicolumn{2}{c}{63.07} & 
% \multicolumn{2}{c}{64.07} &   
% \multicolumn{2}{c}{60.7} &
% \multicolumn{2}{c}{63.73} &
% \multicolumn{2}{c}{\textbf{64.79}} & 
% \multicolumn{2}{c}{63.41} &   
% \multicolumn{2}{c}{64.01} &
% \multicolumn{2}{c}{65.37} & 
% \multicolumn{2}{c}{\textbf{64.83}} &   
% \multicolumn{2}{c}{61.21} 
% \\ 
% \end{tabular}
\end{center}
\caption{\label{table:sur_test} Evaluation of SUR models on 600 test episodes from MetaDataset. Columns: \emph{SUR} shows baseline performance using original  backbones.  \emph{Blur skip}: shows the effect of adding blur to skip connections with various blur kernel size ($k$), \emph{GELU}: replaces ReLU actions with GELU in all backbones, \emph{Blur all + GELU}: backbones includes blur filters at all subsampled modules, and GELU activations and finally \emph{Blur skip + GELU}: includes blur filters at strided-skip connections and GELU activations. 
Anti-aliased architectures used stride 1 in first convolutional layer.
Conclusions: adding blur at skip connections improves performance with or without GELU activations. GELU actions improve performance on their own. The best result is achieved by combining blur on skip connections with GELU activations.}
\end{table*}
}

%Improving SUR original baseline by the use of smooth activation; Adding anti-alias to sub-sampled layers; anti-alias combined with smooth activation We see that using the ``Blur skip'' anti-aliasing improves the performance of ResNet-18, whether using standard activation functions (SUR) or a smooth version of the ReLU (GELU). Perhaps surprisingly, we also see that, in itself, GELU improves the performance on unseen datasets compared to SUR. To our knowledge, this impact of GELU on meta-dataset had not been observed before.}
